CREIMBO: Cross-Regional Ensemble Interactions in Multi-view Brain Observations

Modern recordings of neural activity provide diverse observations of neurons across brain areas, conditions, and subjects; presenting an exciting opportunity to reveal the fundamentals of brain-wide dynamics. Current analysis methods often fail to harness the richness of such data, as they provide either uninterpretable representations or oversimplify models (e.g., by assuming stationary dynamics). Here, instead of regarding asynchronous neural recordings that lack alignment in neural identity or brain areas as a limitation, we leverage these diverse views into the brain to learn a unified model of neural dynamics. We assume that brain activity is driven by multiple hidden global sub-circuits. These sub-circuits represent global basis interactions between neural ensembles -- functional groups of neurons -- such that the time-varying decomposition of these circuits defines how the ensembles' interactions evolve over time non-stationarily. We discover the neural ensembles underlying non-simultaneous observations, along with their non-stationary evolving interactions, with our new model, CREIMBO. CREIMBO identifies the hidden composition of per-session neural ensembles through graph-driven dictionary learning and models the ensemble dynamics on a low-dimensional manifold spanned by a sparse time-varying composition of the global sub-circuits. Thus, CREIMBO disentangles overlapping temporal neural processes while preserving interpretability due to the use of a shared underlying sub-circuit basis. Moreover, CREIMBO distinguishes session-specific computations from global (session-invariant) ones by identifying session covariates and variations in sub-circuit activations. We demonstrate CREIMBO's ability to recover true components in synthetic data, and uncover meaningful brain dynamics including cross-subject neural mechanisms and inter- vs. intra-region dynamical motifs.

==> inputs/figures_to_check.tex <==


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.99\textwidth]{FIGURES/synthetic_results_fig/supp_synthetic_data_complex5.png}
%     % find the slides in E:\ALL_PHD_MATERIALS\CODES\dLDS-multi-regional\PRESENTATIONS
%     %  draft_figures
%     % 


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.99\textwidth]{FIGURES/synthetic_results_fig/supp_masks_simple_synth.png}
%     % find the slides in E:\ALL_PHD_MATERIALS\CODES\dLDS-multi-regional\PRESENTATIONS
%     %  draft_figures
%     % 
% \caption{    CHECK
%     }
%     \label{fig:different_systems}
% \end{figure}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.99\textwidth]{FIGURES/draft_figures/draft_data_vis_for_human2.PNG}
%     % find the slides in E:\ALL_PHD_MATERIALS\CODES\dLDS-multi-regional\PRESENTATIONS
%     %  draft_figures
%     % 
% \caption{Properties of real human neural recordings from~\cite{kyzar2024dataset}.
%     \textbf{A:} Number of neurons per area and per session.
%     \textbf{B:} Average number of neurons per area across sessions, including the standard error. 
%     \textbf{C:} Total number of neurons per session. 
%     \textbf{D:} Number of sessions in which each region appears.
%     \textbf{E:} Number of unique regions present in each session.
% \NMNM{THINGS TO CHANGE: 1) increase numbers in A. 2) change xticks in A to session 1 .. session 2. 3) in C change to the total number of neurons per session instead of 
% the avg. 4) create D, E, F. 5) make C stacked bar on each other
% }    
%     }
%     \label{fig:human_vis}
% \end{figure}



% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{FIGURES/draft_figures/demo_results_human_data.PNG}
%     \caption{Results on human data. }
%     \label{fig:demo_results_human_data}
% \end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{FIGURES/different_fs_interactions.png}
%     \caption{}
%     \label{fig:unregLorenzColor}
% \end{figure}



% \begin{figure}[t]
%     \centering
%     %regions_distributions_final_bar2
%     % 'E:\\ALL_PHD_MATERIALS\\CODES\\dLDS-multi-regional\\FROM_DANDI_SERVER\\explore_regional_results_from_google_drivve.ipynb'
%     % neural_counts_for_subjects Figure(2880x720) E:\ALL_PHD_MATERIALS\CODES\dLDS-multi-regional\human_data_from_colab\figures
%     \includegraphics[width=\textwidth]{FIGURES/supp_human/regions_distributions_final_bar_stars8.png}
%     \caption{Areas distribution in real world human neural data.}
%     \label{fig:synth_fig}
% \end{figure}





% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\textwidth]{FIGURES/supp_human/res1_real_data6.png}
%     % find the slides in E:\ALL_PHD_MATERIALS\CODES\dLDS-multi-regional\PRESENTATIONS\SUPP_FIGURES
%     %  E:\ALL_PHD_MATERIALS\CODES\dLDS-multi-regional\human_data_just_plot_selected.ipynb
% \caption{    
%     }
%     \label{fig:results_D_y_f_full_letters}
% \end{figure}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SYNTHETIC DATA FIGURES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








\begin{figure}[t]
    \centering
    %regions_distributions_final_bar2
    % 'E:\\ALL_PHD_MATERIALS\\CODES\\dLDS-multi-regional\\FROM_DANDI_SERVER\\explore_regional_results_from_google_drivve.ipynb'
    % neural_counts_for_subjects Figure(2880x720) E:\ALL_PHD_MATERIALS\CODES\dLDS-multi-regional\human_data_from_colab\figures
    \includegraphics[width=\textwidth]{FIGURES/synthetic_multi_ensemble/new_synthetic_data_figure_multi_ens2.png}
    \caption{Multi-ensemble synthetic data.\NMNM{FOR REBUTTAL}}
    \label{fig:synth_fig}
\end{figure}




==> inputs/future_things.tex <==
\subsubsection*{Emerging sub-circuits and Cross-session controlled variability}\label{sec:Emerging}
\textbf{Emerging sub-Circuits:} One extension of CREIMBO is the identification of sub-circuits that are specific to a subject, state, or session and emerge uniquely within those conditions. Particularly in scenarios where subject-specific sub-circuits are anticipated alongside global sub-circuits, it is advantageous to enable 'emerging' subcircuits tailored to each subject or session. This approach results in a per-session set of basis operators that
${\bm{f}_k}_{k=1}^K
 = {\bm{f}_k}_{k=1}^{k_\textrm{global}} + \{\bm{f}_k\}^{k_\textrm{global} + k_\textrm{specific}}_{k={k_\textrm{global}}}
$
where $ {\bm{f}_k}_{k=1}^{k_\textrm{global}}$ are shared global sub-circuits (session invariant), and 
$
\bm{f}_k\}^{k_\textrm{global} + k_\textrm{specific}}_{k={k_\textrm{global}}}
$
are session-specific or subject-specific circuits. 


%\subsubsection*{}\label{sec:Cross}
\textbf{Cross-session controlled variability:} Another extension we introduce includes support for controlled, subtle variations in the basic operators across sessions or other labeled states. Specifically, consider a scenario where interactions among subjects are generally similar, but in one subject, the effect of ensemble A on ensemble B is more pronounced due to heightened sensitivity to that particular issue. To accurately capture this phenomenon, we propose the inclusion of a mechanism that accounts for controlled variability in cross-session sub-circuits. This is achieved by adding the sum of Frobenius norm distances of the circuits from each session \(d\), given by \( \sum_{d' \neq d}^D \| {\bm{F}^\textrm{all}}^d - {\bm{F}^\textrm{all}}^{d'}\|_F^2\), to Equation~\eqref{eq:F_infer}.


==> inputs/results.tex <==

\section{Results}


==> inputs/supplementary_technical_details.tex <==
\section{Code and Data Sharing}\label{sec:data_code}
The neural data used in this study~\cite{kyzar2024dataset} is publicly available  with License: ``spdx:CC-BY-4.0''. We used version 0.240123.1806 of the data which can be accessed through the DANDI Archive at \url{https://dandiarchive.org/dandiset/000469/0.240123.1806} (Access Information: dandi:OpenAccess). 
The code will be shared on GitHub upon publication. 

\section{Technical Details}\label{sec:technical}
The whole code is written in Python. We utilized the following Python packages along with their respective versions: scipy (1.8.0), matplotlib (3.8.2), numpy (1.23.5), pandas (1.5.0), seaborn (0.11.2), scikit-learn (1.0.2), pylops (1.18.2), and statsmodels (0.13.2), all within a Python 3.10.4 environment. For the $\ell_1$ regularization, we used the ``SPGL1'' solver of pylops~\cite{van2009probing}.  %Sample of the data (e.g. ~5 sessions, with ~400 time points each) can run on a simple desktop machine however higher data might require additional processing. 
During the writing process, we used ChatGPT very sparingly to improve wording and fix grammar mistakes at the word or sentence level.
The synthetic experiment can run locally on a desktop (e.g., simple ASUS machine). However, the robustness tests with hundreds of random repeats and the human data experiments used the entry node with CPUs only of NERSC's ``Perlmutter'' supercomputer. Running time for each synthetic instance ranges from 0.8 to 2 minutes (with the capability to run in parallel). For the human data, processing all 41 sessions with 1000 time points per session (and varying neuron counts as described in the text and figures) takes between 17 to 25 minutes, depending on parameters and result quality.


